Manyfield Inflation in Random Potentials

We construct models of inflation with many randomly interacting fields and use these to study the generation of cosmological observables. We model the potentials as multi-dimensional Gaussian random fields (GRFs) and identify powerful algebraic simplifications that, for the first time, make it possible to access the manyfield limit of inflation in GRF potentials. Focussing on small-field, slow-roll, approximate saddle-point inflation in potentials with structure on sub-Planckian scales, we construct explicit examples involving up to 100 fields and generate statistical ensembles comprising of 164,000 models involving 5 to 50 fields. For the subset of these that support at least sixty e-folds of inflation, we use the 'transport method' and $\delta N$ formalism to determine the predictions for cosmological observables at the end of inflation, including the power spectrum and the local non-Gaussianities of the primordial perturbations. We find three key results: i) Planck compatibility is not rare, but future experiments may rule out this class of models; ii) In the manyfield limit, the predictions from these models agree well with, but are sharper than, previous results derived using potentials constructed through non-equilibrium Random Matrix Theory; iii) Despite substantial multifield effects, non-Gaussianities are typically very small: $f_{\rm nl}^{\rm loc} \ll 1$. We conclude that many of the 'generic predictions' of single-field inflation can be emergent features of complex inflation models.

==> New_Commands.tex <==
\newcommand{\vv}[1]{\mathbf{#1}}​
\newcommand{\vh}[1]{\mathbf{\hat{#1}}}​
\newcommand{\nb}{\mathbf{\nabla}}​
\newcommand{\dv}{\mathbf{\nabla}\cdot}​
\newcommand{\cl}{\mathbf{\nabla}\times}​
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\vvv}{\mathbf{v}}
\newcommand{\vvu}{\mathbf{u}}
\newcommand{\vvx}{\mathbf{x}}
\newcommand{\vvk}{\mathbf{k}} %new
\newcommand{\vvp}{\mathbf{p}} %new
\newcommand{\vvr}{\mathbf{r}}
\newcommand{\vvR}{\mathbf{R}} %new
\newcommand{\vvG}{\mathbf{G}} %new
\newcommand{\mc}[1]{\mathcal{#1}} %new
\newcommand{\vvrd}{\dot{\mathbf{r}}}
\newcommand{\vvrdd}{\ddot{\mathbf{r}}}
\newcommand{\rrd}{\dot{r}}
\newcommand{\rrdd}{\ddot{r}}
\newcommand{\thetad}{\dot{\theta}}
\newcommand{\thetadd}{\ddot{\theta}}
\newcommand{\phid}{\dot{\phi}}
\newcommand{\phidd}{\ddot{\phi}}

\newcommand{\eq}[1]{\begin{equation}{#1}\end{equation}}​
\newcommand\nt{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\mui}{^{\mu}}
\newcommand{\mli}{_{\mu}}
\newcommand{\nui}{^{\nu}}
\newcommand{\nli}{_{\nu}}
\newcommand{\pd}[2]{\frac{\partial {#1}}{\partial {#2}}}​
\newcommand{\td}[2]{\frac{d{#1}}{d{#2}}}​
\newcommand{\spd}[2]{\frac{\partial^2 {#1}}{\partial {#2}^2}}​
\newcommand{\std}[2]{\frac{d^2 {#1}}{d{#2}^2}}​

%\renewcommand{\abstractname}{Introduction}


